SPARQ-SGD: Event-Triggered and Compressed Communication in Decentralized Stochastic Optimization

In this paper, we propose and analyze SPARQ-SGD, which is an event-triggered and compressed algorithm for decentralized training of large-scale machine learning models. Each node can locally compute a condition (event) which triggers a communication where quantized and sparsified local model parameters are sent. In SPARQ-SGD each node takes at least a fixed number ($H$) of local gradient steps and then checks if the model parameters have significantly changed compared to its last update; it communicates further compressed model parameters only when there is a significant change, as specified by a (design) criterion. We prove that the SPARQ-SGD converges as $O(\frac{1}{nT})$ and $O(\frac{1}{\sqrt{nT}})$ in the strongly-convex and non-convex settings, respectively, demonstrating that such aggressive compression, including event-triggered communication, model sparsification and quantization does not affect the overall convergence rate as compared to uncompressed decentralized training; thereby theoretically yielding communication efficiency for "free". We evaluate SPARQ-SGD over real datasets to demonstrate significant amount of savings in communication over the state-of-the-art.

==> related-work.tex <==
\paragraph{Related work.}
Distributed Stochastic Gradient Descent (SGD) methods have become ubiquitous in training of large scale machine learning models where workers perform computations in parallel and exchange gradients with each other or coordinate with a central server to facilitate parameter updates. This may impose significant communication load on the central server if the number of workers is large, thus there has been recent interest in understanding SGD for \textit{decentralized} setting \cite{lian2017can}, \cite{lian2017asynchronous}, \cite{jiang2017collaborative}. As exchange of full precision gradients is usually prohibitive due to high communication cost in many application like \textit{Federated Learning} (\cite{mcmahan2016communication}, \cite{konevcny2016federated}), compression techniques for communication efficient gradient methods have received great interest.
	\cite{alistarh-qsgd-17}, \cite{teertha}, \cite{terngrad} propose and analyze unbiased stochastic quantizers for gradient compression. Biased compression operators like retaining just Top-K components of gradient have been studied in \cite{AjiHeafield17}, \cite{stich_sparsified_2018}, \cite{alistarh_convergence_2018}, while operations like retaining just sign (and possibly norm) of gradient values have been analyzed in \cite{bernstein2018signsgd}, \cite{stich-signsgd-19}. An alternate approach to saving on communication is to communicate less frequently by performing local SGD iterations instead of communicating in every iteration \cite{stich_local_2018}, \cite{alibaba_local}. A combination of both aggressive gradient compression (possibly biased) and local SGD iterations was analyzed in \cite{basu_qsparse-local-sgd:_2019} for the distributed setting. In decentralized setting, \cite{reisizadeh2018quantized}, \cite{Tong_decentralized18} propose using unbiased stochastic compression for gradient exchange. \cite{assran2018stochastic}, \cite{tatarenko2017non} analyze Stochastic Gradient Push algorithm for non convex objectives which approximates distributed averaging instead of compressing the gradients. More recently, \cite{koloskova_decentralized_2019-1}, \cite{koloskova_decentralized_2019} propose CHOCO-SGD which supports biased compression operators and allows for arbitrary compression precision. Our work most closely relates to this and builds up on it by introducing \textit{event triggered} communication in which we combine local SGD iterations followed by a triggering rule to significantly reduce communication. The idea of event-triggered communication has been explored previously in the control community \cite{Paulo-event-triggered12,distri-event-triggered12,event-triggered-consensus13,dynamic-event-triggered15}, \cite{liu2017asynchronous} and in optimization literature \cite{convex-optimize-event15,event-gradient-sum-consensus16,optimize-dynamic-event-triggered18,optimize-2ndorder-dynamic-event-triggered18}. While existing approaches in these papers focus on continuous-time, deterministic optimization algorithms for convex problems, here we are concerned with discrete-time, stochastic gradient descent algorithms for both convex and non-convex problems.  
\cite{chen2018lag} propose an adaptive scheme to skip gradient computations in a distributed setting for deterministic gradients. As per our knowledge, our method combining compressed communication with event based triggering for decentralized SGD is novel and provides significant savings in communication compared to the state-of-the-art schemes in this area.



==> setup.tex <==

We now establish the notation which would be used throughout the paper.

\begin{itemize}
	\item Consider a graph $G=(V,E)$ with $|V| = n$ nodes. Let the objectives defined by local data on each node be given by $f_i : \mathbb{R}^d \rightarrow \mathbb{R}$ for $i \in [n]$. We consider optimization problems of the form:
	\begin{align*}
	f^* = \min_{x \in \mathbb{R}^d} \left[ f(x) := \frac{1}{n} \sum_{i=1}^{n} f_i(x)   \right]
	\end{align*}
	\item The communication weights are defined by the connectivity matrix $W \in \mathbb{R}^{n \times n} $ having entries $w_{ij}: i,j \in [n] $. $W$ is assumed to be symmetric and doubly stoachstic with spectral gap defined as $$ \delta := 1- | \lambda_2(W) |  $$
	where $1 = | \lambda_1(W) |> | \lambda_2(W) | \geq \hdots \geq | \lambda_n(W) |$ are the eigenvalues of $W$. It is know that simple matrices $W$ with $\delta >0$ exist for every connected graph (\cite{koloskova_decentralized_2019-1}).
	\item Each node performs local SGD iterations followed by a concensus step similar to  (\cite{koloskova_decentralized_2019-1}) and communicate only when the gradient step and the estimate differ substantially. This is highlighted in Algorithm 1 and 2.
\end{itemize}
%---------------------------------
%------------------------------------------------------------------

==> suppl_dec_sgd.tex <==

We restate the sequence of updates for Algorithm \ref{alg_dec_sgd} in matrix form for reference (see Remark \ref{mat_not}):
\begin{align*}
X^{(t+\frac{1}{2})} & = X^{(t)} - \eta_t \partial F(X^{(t)},\xi^{(t)}) \\
\hat{X}^{(t+1)} & = \hat{X}^{{(t)}} + Q((X^{{(t+\frac{1}{2})}} - \hat{X}^{{(t)}})P^{(t)} ) \\
X^{{(t+1)}} & = X^{{(t+\frac{1}{2})}} + \gamma\hat{X}^{{(t+1)}}(W-I) 
\end{align*}
$P^{(t)} \in \mathbb{R}^{n \times n} $ is a diagonal matrix with entry $1$ for nodes that communicate in time step $t$ with regard to the triggering condition and entry 0 for nodes which don't. \\
These equalities are used throughout the proofs in this section. % \\ \\ 
%We first note the following Lemma which is useful in proofs for Theorem \ref{thm_cvx}, Theorem \ref{thm_noncvx_var} and Theorem \ref{thm_noncvx_fix}
%------------Lemma-------
\subsection{Proof of Lemma \ref{lem_dec_sgd}} \label{proof_lem_dec_sgd}
\begin{lemma*} (Restating Lemma \ref{lem_dec_sgd} )
	Consider the sequence of updates as in Algorithm \ref{alg_dec_sgd} with $\eta_t = \frac{b}{a+t } $ (where $a \geq \frac{5}{p}, \, b > 0$) as the learning rate.
%	\begin{align*}
%	X^{(t+\frac{1}{2})} = X^{(t)} - \eta_t \partial F(X^{(t)},\xi^{(t)}) \\
%	\hat{X}^{(t+1)} = \hat{X}^{{(t)}} + Q((X^{{(t+\frac{1}{2})}} - \hat{X}^{{(t)}})P^{(t)} ) \\
%	X^{{(t+1)}} = X^{{(t+\frac{1}{2})}} + \gamma\hat{X}^{{(t+1)}}(W-I) 
%	\end{align*}
%	where $P^{(t)}$ is a diagonal matrix with entry $1$ for nodes that communicate in time step $t$ with regard to the triggering condition.
	Then we have:
	\begin{align*}
	\mathbb{E}\sum_{j=1}^n \Vert \bar{x}_{t} - x_t^{(j)} \Vert^2 = \mathbb{E}\Vert\Bar{X}^{{(t)}} - X^{{(t)}}\Vert_F^2 \leq \frac{20A\eta_{{t}}^2}{p^2}
	\end{align*}
	where $p = \frac{\delta^2 \omega}{644} $, $\delta := 1 - | \lambda_2(W)|$, $\omega$ is contraction parameter for quantization operator $Q$ and  $A=2nG^2 + \frac{p}{2} \left(\frac{8nG^2}{\omega} + \frac{5\omega n c_0}{4} \right) $
\end{lemma*}
\begin{proof}
	Consider the expression 
	\begin{align} \label{suppl_et_eqn}
		e_{t+1} := \Vert X^{(t+1)} - \Bar{X}^{(t+1)} \Vert_F^2 + \Vert X^{(t+1)} - \hat{X}^{(t+2)} \Vert_F^2
	\end{align}
	The first term of (\ref{suppl_et_eqn}) can be bounded as:
	\begin{align*}
	\Vert X^{(t+1)} - \Bar{X}^{(t+1)} \Vert_F^2 & = \Vert X^{(t+\frac{1}{2})} - \Bar{X}^{(t+1)} + \gamma \hat{X}^{(t+1)} (W-I)  \Vert_F^2 \\
%	\intertext{Using the fact that $\Bar{X}^{(t+1)} = \Bar{X}^{(t+\frac{1}{2})}$ (see Remark 3):}
	& \stackrel{(\ref{mean_seq_iter})}{=} \Vert X^{(t+\frac{1}{2})} - \Bar{X}^{(t+\frac{1}{2})} + \gamma \hat{X}^{(t+1)} (W-I)  \Vert_F^2 \\
	& = \Vert X^{(t+\frac{1}{2})} - \Bar{X}^{(t+\frac{1}{2})} + \gamma ({X}^{(t+\frac{1}{2})} - \Bar{X}^{(t+\frac{1}{2})}) (W-I) + \gamma (\hat{X}^{(t+1)}-X^{(t+\frac{1}{2})}) (W-I)  \Vert_F^2 \\
	& = \Vert (X^{(t+\frac{1}{2})} - \Bar{X}^{(t+\frac{1}{2})})((1-\gamma)I + \gamma W) + \gamma (\hat{X}^{(t+1)}-X^{(t+\frac{1}{2})}) (W-I)  \Vert_F^2 \\
%	\intertext{Using the fact $\Vert A + B \Vert_F^2 \leq (1+\alpha)\Vert A\Vert_F^2 + (1+\alpha^{-1})\Vert B \Vert_F^2$ for any $\alpha >0$, }
	& \stackrel{(\ref{bound_l2_sum})}{\leq} (1+\alpha_1)\Vert (X^{(t+\frac{1}{2})} - \Bar{X}^{(t+\frac{1}{2})})((1-\gamma)I + \gamma W)\Vert_F^2 + (1+\alpha_1^{-1}) \Vert \gamma (\hat{X}^{(t+1)}-X^{(t+\frac{1}{2})}) (W-I)  \Vert_F^2 \\
%	\intertext{Using the fact that for any $A \in \mathbb{R}^{d \times n},B \in \mathbb{R}^{n \times n}$, $\Vert AB \Vert_F \leq \Vert A \Vert_F \Vert B\Vert_2$, }
	& \stackrel{(\ref{bound_frob_mult})}{\leq} (1+\alpha_1)\Vert (X^{(t+\frac{1}{2})} - \Bar{X}^{(t+\frac{1}{2})})((1-\gamma)I + \gamma W)\Vert_F^2 + (1+\alpha_1^{-1}) \gamma^2 \Vert  (\hat{X}^{(t+1)}-X^{(t+\frac{1}{2})})\Vert_F^2 .\Vert(W-I) \Vert_2^2 
	\end{align*}
	The first term can be bounded as:
	\begin{align*}
	\Vert (X^{(t+\frac{1}{2})} - \Bar{X}^{(t+\frac{1}{2})})((1-\gamma)I + \gamma W)\Vert_F & \leq (1-\gamma)\Vert X^{(t+\frac{1}{2})} - \Bar{X}^{(t+\frac{1}{2})} \Vert_F + \gamma \Vert (X^{(t+\frac{1}{2})} - \Bar{X}^{(t+\frac{1}{2})} )W\Vert_F \\ 
%	\intertext{Using the definition for $\bar{X}^{(t+\frac{1}{2})} = X^{(t+\frac{1}{2})}\frac{\mathbbm{1}\mathbbm{1}^T}{n} $}
	& \stackrel{(\ref{mean_prop})}{=} (1-\gamma)\Vert X^{(t+\frac{1}{2})} - \Bar{X}^{(t+\frac{1}{2})} \Vert_F + \gamma \left\Vert (X^{(t+\frac{1}{2})} - \Bar{X}^{(t+\frac{1}{2})})\left (W - \frac{\mathbbm{1}\mathbbm{1}^T}{n} \right) \right\Vert_F \\
%	\intertext{Using remark 4,}
	& \stackrel{(\ref{bound_frob_mult}),(\ref{bound_W_mat})}{\leq} (1-\gamma) \Vert X^{(t+\frac{1}{2})} - \Bar{X}^{(t+\frac{1}{2})} \Vert_F + \gamma \Vert X^{(t+\frac{1}{2})} - \Bar{X}^{(t+\frac{1}{2})} \Vert_F (1-\delta) \\
	& =(1-\gamma \delta) \Vert X^{(t+\frac{1}{2})} - \Bar{X}^{(t+\frac{1}{2})} \Vert_F
	\end{align*}
	Substituting above and using $\beta = \text{max}_i \{ 1- \lambda_i(W) \} \Rightarrow \Vert W-I \Vert_2^2 \leq \beta^2 $, we get:
	\begin{align*}
	\Vert X^{(t+1)} - \Bar{X}^{(t+1)} \Vert_F^2 \leq (1+\alpha_1)(1-\gamma \delta)^2 \Vert X^{(t+\frac{1}{2})} - \Bar{X}^{(t+\frac{1}{2})} \Vert_F^2 + (1+\alpha_1^{-1}) \gamma^2 \beta^2  \Vert  {X}^{(t+\frac{1}{2})}-\hat{X}^{(t+1)}\Vert_F^2
	\end{align*}
	Taking expectation w.r.t the entire process, we get:
	\begin{align} \label{suppl_et_eqn_t1}
	\mathbb{E} \Vert X^{(t+1)} - \Bar{X}^{(t+1)} \Vert_F^2 \leq (1+\alpha_1)(1-\gamma \delta)^2 \mathbb{E} \Vert X^{(t+\frac{1}{2})} - \Bar{X}^{(t+\frac{1}{2})} \Vert_F^2 + (1+\alpha_1^{-1}) \gamma^2 \beta^2 \mathbb{E} \Vert  {X}^{(t+\frac{1}{2})}-\hat{X}^{(t+1)}\Vert_F^2
	\end{align}
	Consider the second term in (\ref{suppl_et_eqn}) and take expectation w.r.t entire process:
	\begin{align*}
	\mathbb{E} \Vert X^{(t+1)} - \hat{X}^{(t+2)}\Vert_F^2 & = \mathbb{E} \Vert X^{(t+1)} - \hat{X}^{(t+1)} - Q ( (X^{(t+\frac{3}{2})} - \hat{X}^{(t+1)}) P^{(t+1)} )\Vert_F^2 \\
	& = \mathbb{E} \Vert X^{(t+\frac{3}{2})} - \hat{X}^{(t+1)}+ X^{(t+1)} - X^{(t+\frac{3}{2})} - Q ( (X^{(t+\frac{3}{2})} - \hat{X}^{(t+1)}) P^{(t+1)} )\Vert_F^2 \\
%	\intertext{For any constant $\alpha_2 > 0$,}
	& \stackrel{(\ref{bound_l2_sum})}{\leq}  (1+\alpha_2) \mathbb{E} \Vert X^{(t+\frac{3}{2})} - \hat{X}^{(t+1)} - Q ( (X^{(t+\frac{3}{2})} - \hat{X}^{(t+1)}) P^{(t+1)} )\Vert_F^2 + (1+\alpha_2^{-1})\mathbb{E}\Vert X^{(t+1)} - X^{(t+\frac{3}{2})} \Vert_F^2 \\
	& = (1+\alpha_2) \mathbb{E} \Vert X^{(t+\frac{3}{2})} - \hat{X}^{(t+1)} - Q ( (X^{(t+\frac{3}{2})} - \hat{X}^{(t+1)}) P^{(t+1)} )\Vert_F^2 + (1+\alpha_2^{-1})\mathbb{E}\Vert \eta_{t+1} \partial F (X^{(t+1)}, \xi^{(t+1)}) \Vert_F^2 \\
	& \stackrel{ (\ref{bound_grad})}{\leq} (1+\alpha_2) \mathbb{E} \Vert X^{(t+\frac{3}{2})} - \hat{X}^{(t+1)} - Q ( (X^{(t+\frac{3}{2})} - \hat{X}^{(t+1)}) P^{(t+1)} )\Vert_F^2 + (1+\alpha_2^{-1}) \eta_{t+1}^2nG^2 \\
	& = (1+\alpha_2)  \mathbb{E} \Vert (X^{(t+\frac{3}{2})} - \hat{X}^{(t+1)})P^{(t+1)} - Q ( (X^{(t+\frac{3}{2})} - \hat{X}^{(t+1)}) P^{(t+1)} )\Vert_F^2  \\
	&  \hspace{2cm} + (1+\alpha_2) \mathbb{E} \Vert (X^{(t+\frac{3}{2})} - \hat{X}^{(t+1)})(I - P^{(t+1)})\Vert_F^2  + (1+\alpha_2^{-1}) \eta_{t+1}^2nG^2 \\
%	\intertext{Using the compression property of operator $Q$, }
	& \stackrel{(\ref{bound_comp})}{\leq} (1+\alpha_2) \mathbb{E} \left[(1-\omega) \Vert (X^{(t+\frac{3}{2})} - \hat{X}^{(t+1)})P^{(t+1)} \Vert_F^2 +  \Vert (X^{(t+\frac{3}{2})} - \hat{X}^{(t+1)})(I - P^{(t+1)})\Vert_F^2 \right] \\
	& \hspace{2cm} + (1+\alpha_2^{-1}) \eta_{t+1}^2nG^2  
	\intertext{Adding and subtracting $ (1+\alpha_2)(1-\omega) \mathbb{E} \Vert (X^{(t+\frac{3}{2})} - \hat{X}^{(t+1)})(I - P^{(t+1)})\Vert_F^2$,}
	& = (1+\alpha_2) \mathbb{E} \left[ (1-\omega)  \Vert X^{(t+\frac{3}{2})} - \hat{X}^{(t+1)} \Vert_F^2 + \omega  \Vert (X^{(t+\frac{3}{2})} - \hat{X}^{(t+1)})(I - P^{(t+1)})\Vert_F^2 \right] + (1+\alpha_2^{-1}) \eta_{t+1}^2nG^2 \\
%	\end{align*}
%	The second term in above expresison (multiplied by $(I - P^{(t+1)})$ ) denotes the norm of nodes which did not communicate in timestep $(t+1)$ and thus should be bounded by the triggering condition:
%	\begin{align}
	& \stackrel{(\ref{bound_trig})}{\leq} (1+\alpha_2) (1-\omega) \mathbb{E} \Vert X^{(t+\frac{3}{2})} - \hat{X}^{(t+1)} \Vert_F^2 +(1+\alpha_2)\omega n c_0 \eta_{t+1}^2  + (1+\alpha_2^{-1}) \eta_{t+1}^2nG^2  \\
	& = (1+\alpha_2) (1-\omega) \mathbb{E} \Vert X^{(t+1)}  - \eta_{t+1} \partial F(X^{(t+1)},\xi^{(t+1)}) -  \hat{X}^{(t+1)} \Vert_F^2 + (1+\alpha_2)\omega n c_0 \eta_{t+1}^2 \\
	& \hspace{2cm} + (1+\alpha_2^{-1}) \eta_{t+1}^2nG^2 \\
%	\intertext{For any constant $\alpha_3 > 0$, we have:}
	& \stackrel{(\ref{bound_l2_sum})}{\leq} (1+\alpha_3) (1+\alpha_2) (1-\omega) \mathbb{E} \Vert X^{(t+1)}  -  \hat{X}^{(t+1)} \Vert_F^2 +  (1+\alpha_3^{-1}) (1+\alpha_2) (1-\omega) \mathbb{E} \Vert \eta_{t+1} \partial F(X^{(t+1)},\xi^{(t+1)}) \Vert_F^2 \\
	& \hspace{2cm}+ (1+\alpha_2)\omega n c_0 \eta_{t+1}^2 + (1+\alpha_2^{-1}) \eta_{t+1}^2nG^2 \\
	& \stackrel{( \ref{bound_grad})}{\leq} (1+\alpha_3) (1+\alpha_2) (1-\omega) \mathbb{E} \Vert X^{(t+1)}  -  \hat{X}^{(t+1)} \Vert_F^2 +  (1+\alpha_3^{-1}) (1+\alpha_2) (1-\omega) \eta_{t+1}^2 nG^2 \\
	& \hspace{2cm}+ (1+\alpha_2)\omega n c_0 \eta_{t+1}^2 + (1+\alpha_2^{-1}) \eta_{t+1}^2nG^2 \\
	& = (1+\alpha_3) (1+\alpha_2) (1-\omega) \mathbb{E} \Vert X^{(t+\frac{1}{2})} + \gamma \hat{X}^{(t+1)} (W-I)  -  \hat{X}^{(t+1)} \Vert_F^2 +  (1+\alpha_3^{-1}) (1+\alpha_2) (1-\omega) \eta_{t+1}^2 nG^2 \\
	& \hspace{2cm} + (1+\alpha_2)\omega n c_0 \eta_{t+1}^2 + (1+\alpha_2^{-1}) \eta_{t+1}^2nG^2 \\
%	\intertext{Using Remark 3 (specifically,  $\Bar{X}^{(t+\frac{1}{2})}(W-I) = 0$),}
	& \stackrel{(\ref{mean_prop})}{=} (1+\alpha_3) (1+\alpha_2) (1-\omega)\mathbb{E} \Vert (X^{(t+\frac{1}{2})} - \hat{X}^{(t+1)})((1+\gamma)I - \gamma W) + \gamma (X^{(t+\frac{1}{2})}- \Bar{X}^{(t+\frac{1}{2})})(W-I) \Vert_F^2 \\
	& \hspace{2cm} +  (1+\alpha_3^{-1}) (1+\alpha_2) (1-\omega) \eta_{t+1}^2 nG^2 + (1+\alpha_2)\omega n c_0 \eta_{t+1}^2 + (1+\alpha_2^{-1}) \eta_{t+1}^2nG^2 \\
%	\intertext{For any $\alpha_4 > 0 $, we have:}
	&\stackrel{(\ref{bound_l2_sum})}{ \leq} (1+\alpha_4) (1+\alpha_3) (1+\alpha_2) (1-\omega) \mathbb{E} \Vert (X^{(t+\frac{1}{2})} - \hat{X}^{(t+1)})((1+\gamma)I - \gamma W) \Vert_F^2 \\
	& \hspace{1cm} + (1+\alpha_4^{-1}) (1+\alpha_3) (1+\alpha_2) (1-\omega) \mathbb{E} \Vert \gamma (X^{(t+\frac{1}{2})}- \Bar{X}^{(t+\frac{1}{2})})(W-I) \Vert_F^2 \\
	& \hspace{2cm} +  (1+\alpha_3^{-1}) (1+\alpha_2) (1-\omega) \eta_{t+1}^2 nG^2 + (1+\alpha_2)\omega n c_0 \eta_{t+1}^2 + (1+\alpha_2^{-1}) \eta_{t+1}^2nG^2 
	\end{align*}
	Using $\Vert (1+\gamma)I - \gamma W \Vert_2 = \Vert I + \gamma (I - W) \Vert_2 = 1 +  \gamma \Vert I-W \Vert_2  = 1 + \gamma \beta $ (by definition of $\beta = \text{max}_i \{ 1- \lambda_i(W) \}$) and (\ref{bound_frob_mult}):
	\begin{align} \label{suppl_et_eqn_t2}
	& \leq (1+\gamma \beta )^2 (1+\alpha_4) (1+\alpha_3) (1+\alpha_2) (1-\omega)\mathbb{E} \Vert X^{(t+\frac{1}{2})} - \hat{X}^{(t+1)}\Vert_F^2 \notag \\
	& \hspace{1cm} + \gamma^2 \beta^2 (1+\alpha_4^{-1}) (1+\alpha_3) (1+\alpha_2) (1-\omega) \mathbb{E} \Vert X^{(t+\frac{1}{2})}- \Bar{X}^{(t+\frac{1}{2})} \Vert_F^2 \notag \\
	& \hspace{1cm} +  (1+\alpha_3^{-1}) (1+\alpha_2) (1-\omega) \eta_{t+1}^2 nG^2 + (1+\alpha_2)\omega n c_0 \eta_{t+1}^2 + (1+\alpha_2^{-1}) \eta_{t+1}^2nG^2 
	\end{align}
	Thus combining the bounds for the first (\ref{suppl_et_eqn_t1}) and second (\ref{suppl_et_eqn_t2}) term of $\mathbb{E}[e_{t+1}]$ , we get:
	\begin{align} \label{suppl_et_eqn_total}
	\mathbb{E} [e_{t+1}] & = \mathbb{E} \Vert X^{(t+1)} - \Bar{X} \Vert_F^2 + \mathbb{E} \Vert X^{(t+1)} - \hat{X}^{(t+2)} \Vert_F^2  \notag \\ 
	& \leq (1+\alpha_1)(1-\gamma \delta)^2 \mathbb{E}\Vert X^{(t+\frac{1}{2})} - \Bar{X}^{(t+\frac{1}{2})} \Vert_F^2 + (1+\alpha_1^{-1}) \gamma^2 \beta^2 \mathbb{E} \Vert  {X}^{(t+\frac{1}{2})}-\hat{X}^{(t+1)}\Vert_F^2 \notag \\ 
	& \hspace{0.5cm} + (1+\gamma \beta )^2 (1+\alpha_4) (1+\alpha_3) (1+\alpha_2) (1-\omega) \mathbb{E} \Vert X^{(t+\frac{1}{2})} - \hat{X}^{(t+1)}\Vert_F^2  \notag \\
	& \hspace{0.5cm} + \gamma^2 \beta^2 (1+\alpha_4^{-1}) (1+\alpha_3) (1+\alpha_2) (1-\omega) \mathbb{E} \Vert X^{(t+\frac{1}{2})}- \Bar{X}^{(t+\frac{1}{2})} \Vert_F^2 +  (1+\alpha_3^{-1}) (1+\alpha_2) (1-\omega) \eta_{t+1}^2 nG^2  \notag \\
	& \hspace{0.5cm}+ (1+\alpha_2)\omega n c_0 \eta_{t+1}^2 + (1+\alpha_2^{-1}) \eta_{t+1}^2nG^2
	\end{align}
	Define the following:
	\begin{align*}
	\pi_1 (\gamma) & := \gamma^2 \beta^2 (1+\alpha_1^{-1}) + (1+\gamma \beta )^2 (1+\alpha_4) (1+\alpha_3) (1+\alpha_2) (1-\omega) \\
	\pi_2 (\gamma) & := (1-\delta \gamma)^2(1+\alpha_1) + \gamma^2 \beta^2 (1+\alpha_4^{-1}) (1+\alpha_3) (1+\alpha_2) (1-\omega) \\
	\pi_3 & := (1+\alpha_3^{-1}) (1+\alpha_2) (1-\omega) nG^2 + (1+\alpha_2)\omega n c_0 + (1+\alpha_2^{-1})nG^2 
	\end{align*}
	Thus the above bound on $\mathbb{E}[e_{t+1}]$ in (\ref{suppl_et_eqn_total}) can be rewritten as:
	\begin{align*}
	\mathbb{E} [e_{t+1}] & \leq \pi_1 (\gamma) \mathbb{E} \Vert {X}^{(t+\frac{1}{2})} - \hat{X}^{(t+1)} \Vert_F^2 + \pi_2 (\gamma) \mathbb{E} \Vert X^{(t+\frac{1}{2})} - \Bar{X}^{(t+\frac{1}{2})} \Vert_F^2 + \pi_3 \eta_{t+1}^2 \\
	& \leq max \{ \pi_1 (\gamma) , \pi_2 (\gamma) \} \, \mathbb{E} \left[ \Vert {X}^{(t+\frac{1}{2})} - \hat{X}^{(t+1)} \Vert_F^2 + \Vert X^{(t+\frac{1}{2})} - \Bar{X}^{(t+\frac{1}{2})} \Vert_F^2 \right] + \pi_3 \eta_{t+1}^2
	\end{align*}
	Calculation of $ max \{ \pi_1 (\gamma) , \pi_2 (\gamma) \}$ and $\pi_3$ is given in Lemma \ref{suppl_lem_coeff_calc}. This yields:
	\begin{align*}
	\mathbb{E}[e_{t+1}] \leq \left( 1 - \frac{\delta^2 \omega}{644} \right) \mathbb{E}  \left[ \Vert {X}^{(t+\frac{1}{2})} - \hat{X}^{(t+1)} \Vert_F^2 + \Vert X^{(t+\frac{1}{2})} - \Bar{X}^{(t+\frac{1}{2})} \Vert_F^2 \right] + \left( \frac{8nG^2}{\omega} + \frac{5\omega n c_0}{4} \right) \eta_t^2
	\end{align*}
	where we've used the fact that $\eta_t \geq \eta_{t+1}$ \\
	Defining $p := \frac{\delta^2\omega}{644}$, $c_1:= \left( \frac{8nG^2}{\omega} + \frac{5\omega n c_0}{4} \right) $ and using defintion of $e_{t+1} =  \left[ \Vert X^{{(t+1)}} - \Bar{X}^{{(t+1)}} \Vert_F^2 + \Vert X^{{(t+1)}} - \hat{X}^{{(t+2)}} \Vert_F^2 \right] $, 
	\begin{align*}
	\mathbb{E} \left[ \Vert X^{{(t+1)}} - \Bar{X}^{{(t+1)}} \Vert_F^2 + \Vert X^{{(t+1)}} - \hat{X}^{{(t+2)}} \Vert_F^2 \right] & \leq (1-p)( \mathbb{E} \Vert X^{{(t+\frac{1}{2})}} - \Bar{X}^{{(t+\frac{1}{2})}} \Vert_F^2 + \mathbb{E}\Vert X^{{(t+\frac{1}{2})}} - \hat{X}^{{(t+1)}} \Vert_F^2 ) + c_1 \eta_t^2
	\end{align*}
	Using the fact that $\Bar{X}^{{(t+\frac{1}{2})}} = \Bar{X}^{{(t)}} - \eta_{t}\partial F(X^{(t)}, \xi^{(t)} )   \frac{\mathbbm{1}\mathbbm{1}^T}{n}  $:
	\begin{align*}
	& = (1-p)\mathbb{E}\left\Vert \Bar{X}^{{(t)}} - X^{{(t)}} -  \eta_{t}\partial F(X^{(t)}, \xi^{(t)} )\left(   \frac{\mathbbm{1}\mathbbm{1}^T}{n} - I \right) \right\Vert_F^2 + (1-p)\mathbb{E}\left\Vert \hat{X}^{{(t+1)}} - X^{{(t)}} + \eta_{t} \partial F(X^{(t)}, \xi^{(t)} )\right\Vert_F^2 + c_1 \eta_t^2 \\
	& \stackrel{(\ref{bound_l2_sum})}{\leq} (1-p)(1+\alpha_1^{-1})\mathbb{E}\left[ \Vert\Bar{X}^{{(t)}} - X^{{(t)}}\Vert_F^2  + \Vert \hat{X}^{{(t+1)}} - X^{{(t)}} \Vert_F^2 \right] + (1-p)(1+\alpha_1) \mathbb{E}\left\Vert \eta_{t}\partial F(X^{(t)}, \xi^{(t)} )\left(   \frac{\mathbbm{1}\mathbbm{1}^T}{n} - I \right) \right\Vert_F^2  \\
	& \hspace{1cm} + (1-p)(1+\alpha_1) \mathbb{E}\left\Vert \eta_{t}\partial F(X^{(t)}, \xi^{(t)} )\right\Vert_F^2 + c_1 \eta_t^2 \\
%	\intertext{Using $\mathbb{E} \left\Vert \eta_{t}\partial F(X^{(t)}, \xi^{(t)} )\right\Vert_F^2  \leq \eta_{{t}} nG^2 $ and $\Vert \frac{\mathbbm{1}\mathbbm{1}^T}{n} - I \Vert_2^2 = 1 $ }
	& \stackrel{(\ref{bound_grad}),(\ref{bound_W_mat})}{\leq} (1-p) (1+\alpha_1^{-1})\mathbb{E}\left[ \Vert\Bar{X}^{{(t)}} - X^{{(t)}}\Vert_F^2  + \Vert \hat{X}^{{(t+1)}} - X^{{(t)}} \Vert_F^2 \right]  + (1-p)(1+\alpha_1) 2G^2n \eta_{t}^2 + c_1 \eta_t^2 \\
%	\intertext{Setting $\alpha_1 = \frac{2}{p}$, we have: }
	&\stackrel{ ( \alpha_1 = \frac{2}{p} ) }{\leq} \left( 1-\frac{p}{2} \right)\mathbb{E}\left[ \Vert\Bar{X}^{{(t)}} - X^{{(t)}}\Vert_F^2  + \Vert \hat{X}^{{(t+1)}} - X^{{(t)}} \Vert_F^2 \right] + \frac{4n}{p}\eta_{t}^2G^2 + c_1 \eta_t^2
	\end{align*}
	Define $A := 2nG^2 + \frac{p c_1}{2}$ (where $c_1= \left( \frac{8nG^2}{\omega} + \frac{5\omega n c_0}{4} \right) $ as above), thus we have the following relation:
	\begin{align*}
	\mathbb{E}\left[\Vert X^{{(t+1)}} - \Bar{X}^{{(t+1)}} \Vert_F^2 + \Vert X^{{(t+1)}} - \hat{X}^{{(t+2)}} \Vert_F^2 \right] \leq \left( 1-\frac{p}{2} \right)\mathbb{E}\left[ \Vert\Bar{X}^{{(t)}} - X^{{(t)}}\Vert_F^2  + \Vert \hat{X}^{{(t+1)}} - X^{{(t)}} \Vert_F^2 \right] + \frac{2A}{p}\eta_{t}^2
	\end{align*}
	Using $e_t : =  \left[ \Vert\Bar{X}^{{(t)}} - X^{{(t)}}\Vert_F^2  + \Vert \hat{X}^{{(t+1)}} - X^{{(t)}} \Vert_F^2 \right] $, above can be written as:
	\begin{align} \label{suppl_lemm_rec_rel}
	\mathbb{E}[e_{t+1}] \leq \left( 1- \frac{p}{2} \right)\mathbb{E}[e_t] + \frac{2A}{p} \eta_t^2
	\end{align}
	Thus, employing Lemma \ref{suppl_lem_e_seq}, the sequence $\mathbb{E}[e_{t}]$ follows the bound for all $t$: 
	\begin{align*}
	\mathbb{E}[e_t] \leq \frac{20A\eta_{{t}}^2}{p^2}
	\end{align*}
	Note that we also have :  $\mathbb{E}\Vert\Bar{X}^{{(t)}} - X^{{(t)}}\Vert_F^2 \leq \mathbb{E} \left[ \Vert\Bar{X}^{{(t)}} - X^{{(t)}}\Vert_F^2  + \Vert \hat{X}^{{(t+1)}} - X^{{(t)}} \Vert_F^2 \right] := \mathbb{E}[e_{t}] $. Thus, we get:
	\begin{align*}
	\mathbb{E}\Vert\Bar{X}^{{(t)}} - X^{{(t)}}\Vert_F^2 \leq \frac{20A\eta_{{t}}^2}{p^2}
	\end{align*}
	where $A := 2nG^2 + \frac{p}{2} \left( \frac{8nG^2}{\omega} + \frac{5 \omega n c_0}{4} \right) $ and $p = \left( 1 - \frac{\delta^2 \omega}{644} \right)$. 
\end{proof}
%------------Lemma-------
\begin{lemma} \label{suppl_lem_coeff_calc}
	Consider:
	\begin{align*}
	\pi_1 (\gamma) & := \gamma^2 \beta^2 (1+\alpha_1^{-1}) + (1+\gamma \beta )^2 (1+\alpha_4) (1+\alpha_3) (1+\alpha_2) (1-\omega) \\
	\pi_2 (\gamma) & := (1-\delta \gamma)^2(1+\alpha_1) + \gamma^2 \beta^2 (1+\alpha_4^{-1}) (1+\alpha_3) (1+\alpha_2) (1-\omega) \\
	\pi_3 & := (1+\alpha_3^{-1}) (1+\alpha_2) (1-\omega) nG^2 + (1+\alpha_2)\omega n c_0 + (1+\alpha_2^{-1})nG^2 
	\end{align*}
	and the following choice of variables:
	\begin{align*}
	\alpha_1 := \frac{\gamma \delta}{2}, \, 
	\alpha_2 := \frac{\omega}{4}, \,
	\alpha_3 := \frac{\omega}{4}, \,
	\alpha_4 := \frac{\omega}{4} \\
	\gamma^* := \frac{2 \delta \omega}{64 \delta + \delta^2 + 16 \beta^2 + 8 \delta \beta^2 - 16\delta \omega} \\
	\end{align*}
	Then, it can be shown that:
	\begin{align*}
	max \{ \pi_1 (\gamma^*) , \pi_2 (\gamma^*) \} & \leq 1 - \frac{\delta^2 \omega}{644} \hspace{0.5cm}, \hspace{0.5cm}
	\pi_3 \leq \frac{8nG^2}{\omega} + \frac{5\omega nc_0}{4}
	\end{align*}
\end{lemma}
\begin{proof}
	Consider:
	\begin{align*}
	(1+\alpha_4) (1+\alpha_3) (1+\alpha_2) (1-\omega) & = (1+\frac{\omega}{4})^3 (1-\omega) \\
	& = \left( 1 - \frac{\omega^4}{64} - \frac{11 \omega^3}{64} - \frac{9 \omega^2}{16} - \frac{\omega}{4} \right) \\
	& \leq \left( 1 - \frac{\omega}{4} \right)
	\end{align*}
	This gives us:
	\begin{align*}
	\pi_1(\gamma) \leq \gamma^2\beta^2\left(1+\frac{2}{\gamma \delta} \right) + (1+\gamma\beta)^2 \left( 1 - \frac{\omega}{4} \right)
	\end{align*}
	Noting that $\gamma^2 \leq \gamma $ (for $\gamma \leq 1 $ which is true for $\gamma^*$ ) and $\beta \leq 2$, we have:
	\begin{align*}
	\pi_1(\gamma) \leq \beta^2\left(\gamma +\frac{2\gamma}{\delta} \right) + (1+8\gamma) \left( 1 - \frac{\omega}{4} \right)
	\end{align*}
	Substituting value of $\gamma^*$ in above, it can be shown that:
	\begin{align*}
	\pi_1(\gamma^*) \leq 1 - \frac{\delta^2\omega}{4(64 \delta + \delta^2 + 16 \beta^2 + 8 \delta \beta^2 - 16\delta \omega)}
	\end{align*}
	Now we note that:
	\begin{align*}
	\pi_2 (\gamma) & =  (1-\delta \gamma)^2 \left(1+\frac{\delta \gamma}{2} \right) + \gamma^2 \beta^2 \left( 1+\frac{4}{\omega} \right) \left(1+\frac{\omega}{4} \right)^2 (1-\omega) 
	\intertext{where we use the fact that for $x = \delta \gamma \leq 1 $ : $\left( 1 - x  \right) \left(1 + \frac{x}{2}\right) \leq \left( 1 - \frac{x}{2}  \right) $ and $ \left( 1 -x \right) \left( 1 - \frac{x}{2} \right) \leq \left( 1 - \frac{x}{2}\right)^2 $ }
	& \leq \left( 1-\frac{\gamma \delta}{2} \right)^2 + \gamma^2 \beta^2 \left( 1+\frac{4}{\omega} \right) \left(1+\frac{\omega}{4} \right)^2 (1-\omega)\\
%	& = \left( 1-\frac{\gamma \delta}{2} \right)^2 + \gamma^2 \beta^2 \left( 1+\frac{4}{\omega} \right) \left(1+\frac{\omega^2}{16} + \frac{\omega}{2} \right) (1-\omega) \\
	& = \left( 1-\frac{\gamma \delta}{2} \right)^2 + \gamma^2 \beta^2 \left(3+\frac{3\omega}{4}+\frac{\omega^2}{16} + \frac{4}{\omega} \right) (1-\omega) \\
	& \leq \left( 1-\frac{\gamma \delta}{2} \right)^2 + \gamma^2 \beta^2 \frac{4}{\omega} \, : = \zeta(\gamma)
	\end{align*}
	Note that $\zeta(\gamma)$ is convex and quadratic in $\gamma$, the minimum value is attained at $\gamma' = \frac{2 \delta \omega}{16 \beta^2 + \delta^2 \omega}$ with value $\zeta(\gamma') = \frac{16\beta^2}{16\beta^2 + \omega \delta^2}$ \\
	By Jensen's inequality, we note that for any $\lambda \in [0,1]$
	\begin{align*}
	\zeta(\lambda \gamma') \leq (1-\lambda) \zeta(0) + \lambda \zeta(\gamma') = 1 - \lambda \frac{\delta^2 \omega}{16 \beta^2 + \delta^2 \omega}
	\end{align*}
	For the choice $\lambda' = \frac{16\beta^2 + \omega \delta^2}{64 \delta + \delta^2 + 16 \beta^2 + 8 \delta \beta^2 - 16\delta \omega}$, it can be seen that $\lambda' \gamma' = \gamma^*$. Thus we get:
	\begin{align*}
	\pi_2(\gamma^*) \leq  \zeta(\lambda' \gamma')  & \leq 1 - \frac{\delta^2\omega}{(64 \delta + \delta^2 + 16 \beta^2 + 8 \delta \beta^2 - 16\delta \omega)} \\
	& \leq 1 - \frac{\delta^2\omega}{4(64 \delta + \delta^2 + 16 \beta^2 + 8 \delta \beta^2 - 16\delta \omega)}
	\end{align*}
	Now we note the value of $\pi_3$ (here $\omega \in (0,1)$):
	\begin{align*}
	\pi_3 & = \left( 1+\frac{4}{\omega} \right)nG^2 + \left( 1 + \frac{\omega}{4} \right) (1 - \omega)\left( 1+\frac{4}{\omega} \right) nG^2 + \left( 1+\frac{\omega}{4} \right)\omega n c_0\\
	& = \left( 1+\frac{4}{\omega} \right) nG^2 \left[ 2 - \frac{3\omega}{4} - \frac{\omega^2}{4} \right] + \left( 1+\frac{\omega}{4} \right)\omega n c_0\\
	& \leq 2nG^2\left( 1+\frac{4}{\omega} \right)\left( 1-\frac{3\omega}{8} \right)+ \frac{5\omega n c_0}{4} = 2nG^2\left( 1-\frac{3\omega}{8} + \frac{4}{\omega} - \frac{3}{2} \right) + \frac{5\omega n c_0}{4} \\
	& \leq \frac{8nG^2}{\omega} + \frac{5\omega n c_0}{4}
	\end{align*}
	Thus we have:
	\begin{align*}
	max \{ \pi_1 (\gamma^*) , \pi_2 (\gamma^*) \} & \leq 1 - \frac{\delta^2\omega}{4(64 \delta + \delta^2 + 16 \beta^2 + 8 \delta \beta^2 - 16\delta \omega)}
	\intertext{Using crude estimates $\delta \leq 1, \omega \geq 0, \beta \leq2, $}
	& \leq 1 - \frac{\delta^2 \omega}{644}
	\end{align*}
\end{proof}
%------------Lemma-------
\begin{lemma} \label{suppl_lem_e_seq}
	Consider the sequence \{$e_{t}$\} given by
	\begin{align*}
	e_{{t+1}} \leq \left( 1-\frac{p}{2} \right)e_{t} + \frac{2}{p}\eta_{t}^2A
	\end{align*}
	For a parameter $p >0$, stepsize $\eta_t = \frac{b}{t+a}$, for parameter $a \geq \frac{5}{p}$ and arbitrary $b >0$, we have:
	\begin{align*}
	e_{t} \leq \frac{20}{p^2}A\eta_{{t}}^2
	\end{align*}
\end{lemma}
\begin{proof}
	We will proceed the proof by induction. Note that for t=0, $e_{0}:=0$, thus statement is true. Assume the statement holds for index $t$, then for index $(t+1)$:  
	\begin{align*}
	e_{{t+1}} \leq \left( 1- \frac{p}{2} \right)e_{{t}} + \frac{2}{p}A\eta_{{t}}^2 \leq  \left( 1- \frac{p}{2} \right)\frac{20}{p^2}A\eta_{{t}}^2 + \frac{2}{p}A\eta_{{t}}^2  = \frac{A\eta_{{t}}^2}{p^2}(20-8p) \stackrel{(p \geq \frac{5}{a})}{\leq} \frac{20A\eta_{{t}}^2}{p^2}\left( 1- \frac{2}{a} \right)  
	\end{align*}
	Now, we note the following:
	\begin{align*}
	(a+ {t+1})^2 \left( 1- \frac{2}{a} \right)     & = (a+ 1)^2 + 2(a+ {t}) + 1 - \left[ \frac{2(a+ {t})^2}{a} + \frac{4(a+ {t})}{a} + \frac{2}{a} \right] \\
	& \leq (a+ {t})^2 + 2(a+ {t}) + 1 - \left[ 2(a+ {t}) + 4 \right] \\
	& \leq (a+ {t})^2
	\end{align*}
	Thus, for $\eta_{{t+1}} = \frac{b}{a + {t+1} }$, we get:
	\begin{align*}
	\eta_{{t}}^2 \left( 1- \frac{2}{a} \right) \leq \eta_{{t+1}}^2
	\end{align*}
	Substituting the above bound in the bound for $e_{t+1}$ gives us:
	\begin{align*}
	e_{{t+1}} \leq \frac{20A\eta_{{t+1}}^2}{p^2}
	\end{align*}
	Thus, by induction : $e_{{t}} \leq \frac{20A\eta_{{t}}^2}{p^2}$ for all $t$.
\end{proof}
%------------------------------------------------------------------
%------------------------------------------------------------------
\subsection{Proof of Theorem \ref{thm_cvx} (Strongly convex objective)} \label{proof_thm_cvx}
%To proceed proving the Theorem, we first note the following lemma:
%------------Lemma-------
%The proof below uses techniques from \cite{stich_sparsified_2018}, \cite{koloskova_decentralized_2019-1}.
%\begin{lemma} \label{suppl_cvx_lemm}
%	 Let $ \{ x_t ^{(i)}  \}_{t=0}^{T-1} $ be generated according to Algorithm \ref{alg_dec_sgd} or Algorithm \ref{alg_dec_sgd_li} with stepsize $\eta_t $ and define $\bar{x}_t = \frac{1}{n} \sum_{i=1}^{n} x_t^{(i)} $. Then we have the following result for $\bar{x}^{(t)}$ :
%	\begin{align*}
%	\mathbb{E}_{\xi_t} \Vert \Bar{x}^{(t+1)} - x^* \Vert^2 \leq & \left( 1-\frac{\eta_t \mu}{2} \right) \Vert \Bar{x}^{(t)} - x^* \Vert^2 + \frac{\eta_t^2 \Bar{\sigma}^2}{n} - 2\eta_t (1-2L\eta_t) (f(\Bar{x}^{(t)}) - f^*)  + \eta_t \left(  \frac{2\eta_t L^2 + L + \mu}{n}  \right) \sum_{j=1}^n \Vert \Bar{x}^{(t)} - x_j^{(t)} \Vert^2
%	\end{align*}
%	where $\xi_t$ is the set of random samples at each worker at time step $t$ : $ \{ \xi_1^{(t)},\xi_2^{(t)}, \hdots, \xi_n^{(t)}  \}$ and $\bar{\sigma}^2 = \frac{1}{n} \sum_{i=1}^{n} \sigma_i^2$
%\end{lemma}
%\begin{proof} Consider expectation taken over sampling at time instant $t$ and using $\Bar{X}^{(t)}  = \Bar{X}^{(t+\frac{1}{2})} $ (from (\ref{mean_seq_iter})  ) ,  we have:
%	\begin{align}
%	\mathbb{E}_{\xi_t} \Vert \Bar{x}^{(t+1)} - x^* \Vert^ 2 & =  \mathbb{E}_{\xi_t} \left\Vert \Bar{x}^{(t)} - \frac{\eta_t}{n}\sum_{j=1}^n \nabla F_j(x_j^{(t)},\xi_j^{(t)}) - x^* \right\Vert^2  \notag\\
%	& = \mathbb{E}_{\xi_t} \left\Vert \Bar{x}^{(t)} - x^* - \frac{\eta_t}{n}\sum_{j=1}^n \nabla f_j(x_j^{(t)}) + \frac{\eta_t}{n}\sum_{j=1}^n \nabla f_j(x_j^{(t)}) - \frac{\eta_t}{n}\sum_{j=1}^n \nabla F_j(x_j^{(t)},\xi_j^{(t)})  \right\Vert^2  \notag\\
%	& =  \left\Vert \Bar{x}^{(t)} - x^* - \frac{\eta_t}{n}\sum_{j=1}^n \nabla f_j(x_j^{(t)}) \right\Vert^2 + \eta_t^2 \mathbb{E}_{\xi_t} \left\Vert \frac{1}{n}\sum_{j=1}^n \nabla f_j(x_j^{(t)}) - \frac{1}{n}\sum_{j=1}^n \nabla F_j(x_j^{(t)},\xi_j^{(t)}) \right\Vert^2 \notag\\
%	& \hspace{1cm} + \frac{2\eta_t}{n}\mathbb{E}_{\xi_t} \left\langle \Bar{x}^{(t)} - x^* - \frac{\eta_t}{n}\sum_{j=1}^n \nabla f_j(x_j^{(t)}) , \sum_{j=1}^n \nabla f_j(x_j^{(t)}) - \sum_{j=1}^n \nabla F_j(x_j^{(t)},\xi_j^{(t)}) \right\rangle \label{suppl_cvx_lemm_total}
%	\end{align}
%	The last term in is zero as $\mathbb{E}_{\xi_i^{(t)}} \nabla F_i(x_i^{(t)}, \xi_i^{(t)}) = \nabla f_i(x_i^{(t)}) $ for all $i \in [n]$. The second term in can be bounded via the variance bound (\ref{bound_var}) by $ \frac{\eta_t^2 \bar{\sigma}^2}{n}$.
%%	\begin{align}
%%	\mathbb{E}_{\xi_t}\left\Vert \frac{1}{n}\sum_{j=1}^n \nabla f_j(x_j^{(t)}) - \frac{1}{n}\sum_{j=1}^n \nabla F_j(x_j^{(t)},\xi_j^{(t)}) \right\Vert^2 & = 
%%	\frac{1}{n^2} \sum_{j=1}^n \mathbb{E}_{\xi_t} \Vert \nabla f_j(x_j^{(t)}) - \nabla F_j(x_j^{(t)},\xi_j^{(t)})\Vert^2 \\
%%	& \hspace{1cm} + \frac{1}{n^2}\sum_{i \neq j} \mathbb{E}_{\xi_t} \left\langle \nabla f_i(x_i^{(t)}) - \nabla F_i(x_i^{(t)},\xi_j^{(t)}), \nabla f_j(x_j^{(t)}) - \nabla F_j(x_j^{(t)},\xi_j^{(t)}) \right\rangle \\
%%	\intertext{Since $\xi_i$ is independent of $\xi_j$, the second term is zero in expectation,}
%%	& = \frac{1}{n^2} \sum_{j=1}^n \mathbb{E}_{\xi_t} \Vert \nabla f_j(x_j^{(t)}) - \nabla F_j(x_j^{(t)},\xi_j^{(t)})\Vert^2 \\
%%	& \leq \frac{1}{n^2} \sum_{j=1}^n \sigma_j^2 = \frac{\Bar{\sigma}^2}{n}
%%	\end{align}
%	We consider the first term in the expression:
%	\begin{align} \label{suppl_cvx_lemm_firstterm}
%	 \left\Vert \Bar{x}^{(t)} - x^* - \frac{\eta_t}{n}\sum_{j=1}^n \nabla f_j(x_j^{(t)}) \right\Vert^2 = \Vert \Bar{x}^{(t)} - x^* \Vert^2 + \eta_t^2  \underbrace{\left\Vert \frac{1}{n}\sum_{j=1}^n \nabla f_j(x_j^{(t)}) \right\Vert^2}_{T_1} - \underbrace{2\eta_t  \left\langle \Bar{x}^{(t)} - x^*,\frac{1}{n}\sum_{j=1}^n \nabla f_j(x_j^{(t)}) \right\rangle}_{T_2}
%	\end{align}
%	Bounding $T_1$ in (\ref{suppl_cvx_lemm_firstterm}) (by noting that $\nabla f_j(x^*) = 0 $ for all $j \in [n]$ ):
%	\begin{align}
%	T_1 &= \left\Vert \frac{1}{n}\sum_{j=1}^n (\nabla f_j(x_j^{(t)}) - \nabla f_j(\Bar{x}^{(t)}) + \nabla f_j(\Bar{x}^{(t)}) - \nabla f_j(x^*) ) \right\Vert^2  \notag \\
%	& \leq \frac{2}{n}\sum_{j=1}^n \Vert \nabla f_j(x_j^{(t)}) - \nabla f_j(\Bar{x}^{(t)}) \Vert^2 + 2 \left\Vert \frac{1}{n}\sum_{j=1}^n \nabla f_j(\Bar{x}^{(t)}) - \frac{1}{n}\sum_{j=1}^n \nabla f_j(x^*) \right\Vert^2  \notag \\
%%	\intertext{Using strong convexity of $f$, optimality of $x^*$ and $L-$smoothness property (\ref{l_smooth_prop}) of $f_j$ , and by noting that  :  $$ \left\Vert \frac{1}{n}\sum_{j=1}^n \nabla f_j(\Bar{x}^{(t)}) - \frac{1}{n}\sum_{j=1}^n \nabla f_j(x^*) \right\Vert^2 \leq \frac{1}{n} \sum_{j=1}^n \Vert \nabla f_j(\Bar{x}^{(t)}) -  \nabla f_j(x^*) \Vert^2  \leq \frac{1}{n} \sum_{j=1}^n 2L (f_j(\Bar{x}^{(t)}) - f_j(x^*)) $$ , }
%	& \stackrel{(a)}{\leq} \frac{2L^2}{n}\sum_{j=1}^n \Vert x_j^{(t)} - \Bar{x}^{(t)} \Vert^2 + \frac{4L}{n} \sum_{j=1}^n (f_j(\Bar{x}^{(t)}) - f_j(x^*))  \notag \label{suppl_cvx_t1_bound} \\
%	& = \frac{2L^2}{n}\sum_{j=1}^n \Vert x_j^{(t)} - \Bar{x}^{(t)} \Vert^2 + 4L  (f(\Bar{x}^{(t)}) - f^*) 
%	\end{align}
%	where in $(a)$, we've used strong convexity of $f$, optimality of $x^*$, $L-$smoothness property (\ref{l_smooth_prop}) of $f_j's$  to bound the first term. The second term is bounded by noting that  :  $$ \left\Vert \frac{1}{n}\sum_{j=1}^n \nabla f_j(\Bar{x}^{(t)}) - \frac{1}{n}\sum_{j=1}^n \nabla f_j(x^*) \right\Vert^2 \leq \frac{1}{n} \sum_{j=1}^n \Vert \nabla f_j(\Bar{x}^{(t)}) -  \nabla f_j(x^*) \Vert^2  \leq \frac{1}{n} \sum_{j=1}^n 2L (f_j(\Bar{x}^{(t)}) - f_j(x^*)) $$
%	Bounding $T_2$ in (\ref{suppl_cvx_lemm_firstterm}):
%	\begin{align}
%	-\frac{1}{\eta_t}T_2 & = -\frac{2}{n} \sum_{j=1}^n \left[ \left\langle \Bar{x}^{(t)} - x_j^{(t)}, \nabla f_j(x_j^{(t)}) \right\rangle + \left\langle x_j^{(t)} - x^*, \nabla f_j(x_j^{(t)}) \right\rangle \right] \notag  \\
%	\intertext{Using expression for $\mu$-strong convexity (\ref{mu_strong_cvx}) and $L$-smoothness (\ref{l_smooth}) for $f_j , \, j \in [n] $  : }
%	& \leq -\frac{2}{n} \sum_{j=1}^n \left[  f_j(\Bar{x}^{(t)}) - f_j(x_j^{(t)}) - \frac{L}{2}\Vert \Bar{x}^{(t)} - x_j^{(t)}  \Vert^2  + f_j(x_j^{(t)}) - f_j(x^*) + \frac{\mu}{2}\Vert x_j^{(t)} - x^*  \Vert^2 \right] \notag \\
%	& \leq  -2  (f(\Bar{x}^{(t)}) - f(x^*)) + \frac{L+ \mu}{n}\sum_{j=1}^n \Vert \Bar{x}^{(t)} - x_j^{(t)}  \Vert^2   - \frac{\mu}{2} \Vert \Bar{x}^{(t)} - x^*  \Vert^2 \label{suppl_cvx_t2_bound}
%	\end{align}
%	Substituting (\ref{suppl_cvx_t1_bound}),(\ref{suppl_cvx_t2_bound}) in (\ref{suppl_cvx_lemm_firstterm}) and using it in (\ref{suppl_cvx_lemm_total}), we get the desired result :
%	\begin{align*}
%	 \mathbb{E}_{\xi_t} \Vert \Bar{x}^{(t+1)} - x^* \Vert^2 \leq \left( 1-\frac{\eta_t \mu}{2} \right) \Vert \Bar{x}^{(t)} - x^* \Vert^2 + \frac{\eta_t^2 \Bar{\sigma}^2}{n} - 2\eta_t (1-2L\eta_t) (f(\Bar{x}^{(t)}) - f^*) + 
%	\eta_t \left(  \frac{2\eta_t L^2 + L + \mu}{n}  \right) \sum_{j=1}^n \Vert \Bar{x}^{(t)} - x_j^{(t)} \Vert^2
%	\end{align*}
%\end{proof}
\begin{proof}[Proof of Theorem ~\ref{thm_cvx}]
	From Lemma \ref{suppl_cvx_lemm}, we have that :
	\begin{align*}
	\mathbb{E}_{\xi_t} \Vert \Bar{x}^{(t+1)} - x^* \Vert^2 \leq \left( 1-\frac{\eta_t \mu}{2} \right) \Vert \Bar{x}^{(t)} - x^* \Vert^2 + \frac{\eta_t^2 \Bar{\sigma}^2}{n} - 2\eta_t (1-2L\eta_t) (f(\Bar{x}^{(t)}) - f^*) + 
	\eta_t \left(  \frac{2\eta_t L^2 + L + \mu}{n}  \right) \sum_{j=1}^n \Vert \Bar{x}^{(t)} - x_j^{(t)} \Vert^2
	\end{align*}
	Taking expecatin w.r.t the whole process gives us:
	\begin{align} \label{suppl_cvx_lemm_use}
	\mathbb{E}\Vert \Bar{x}^{(t+1)} - x^* \Vert^2 \leq \left( 1-\frac{\eta_t \mu}{2} \right) \mathbb{E} \Vert \Bar{x}^{(t)} - x^* \Vert^2 + \frac{\eta_t^2 \Bar{\sigma}^2}{n} - 2\eta_t (1-2L\eta_t) (\mathbb{E}f(\Bar{x}^{(t)}) - f^*) + 
	\eta_t \left(  \frac{2\eta_t L^2 + L + \mu}{n}  \right) \sum_{j=1}^n \mathbb{E}\Vert \Bar{x}^{(t)} - x_j^{(t)} \Vert^2
	\end{align}
	The last term in (\ref{suppl_cvx_lemm_use}), can be bounded by using Lemma \ref{lem_dec_sgd} which gives us:
	%\begin{align}
	%\Gamma_{t} = \sum_{j=1}^n \mathbb{E}\Vert \Bar{x}^{(t)} - x_j^{(t)} \Vert^2 = \mathbb{E} \Vert X^{(t)} - \Bar{X}^{(t)} \Vert_F^2
	%\end{align}
	%Using Lemma0.7, for $A= 2nG^2 + \frac{p}{2}\left( \frac{8nG^2}{\omega} + \frac{5\omega n c_0}{4} \right)$
	%\begin{align}
	%\Gamma_{t} \leq \frac{20A}{p^2} \eta_t^2
	%\end{align}
	%Substituting (92) in (90) (Lemma0.10) yields:
	\begin{align*}
	\mathbb{E} \Vert \Bar{x}^{(t+1)} - x^* \Vert^2 & \leq \left( 1-\frac{\eta_t \mu}{2} \right) \mathbb{E} \Vert \Bar{x}^{(t)} - x^* \Vert^2 + \frac{\eta_t^2 \Bar{\sigma}^2}{n} - 2\eta_t (1-2L\eta_t) (\mathbb{E}f(\Bar{x}^{(t)}) - f^*)  + \eta_t \left(  \frac{2\eta_t L^2 + L + \mu}{n}  \right)\frac{20A}{p^2}\eta_t^2 
	\intertext{where $A= 2nG^2 + \frac{p}{2}\left( \frac{8nG^2}{\omega} + \frac{5\omega n c_0}{4} \right)$}
	& \stackrel{(b)}{\leq} \left( 1-\frac{\eta_t \mu}{2} \right) \mathbb{E} \Vert \Bar{x}^{(t)} - x^* \Vert^2 - \eta_t (\mathbb{E}f(\Bar{x}^{(t)}) - f^*) + \frac{\eta_t^2 \Bar{\sigma}^2}{n}  + \eta_t^3 \left(  \frac{2L + \mu}{n}  \right) \frac{20A}{p^2}
	\end{align*}
	where in $(b)$, we use $a \geq \text{max} \{ \frac{16L}{\mu}, \frac{5}{p}\} $ implying $\eta_t \leq \frac{1}{4L}$ which gives $2L\eta_t - 1 \leq -\frac{1}{2}$ and $(2\eta_t L^2 + L + \mu) \leq (2L + \mu)$ for $\eta_t := \frac{4}{\mu (a+t)}$ \\ 
	%For $\eta_t = \frac{4}{\mu (a+t)}$ and $a \geq \text{max} \{ \frac{16L}{\mu}, \frac{5}{p}\} $, we have $\eta_t \leq \frac{1}{4L}$. This gives:
	%\begin{align*}
	%2L\eta_t - 1 \leq -\frac{1}{2} \\
	%(2\eta_t L^2 + L + \mu) \leq (2L + \mu)
	%\end{align*}
	%Using (95) and (96) in (93-94), we have:
	%\begin{align}
	%\mathbb{E} \Vert \Bar{x}^{(t+1)} - x^* \Vert^2 & \leq \left( 1-\frac{\eta_t \mu}{2} \right) \mathbb{E} \Vert \Bar{x}^{(t)} - x^* \Vert^2 - \eta_t (f(\Bar{x}^{(t)}) - f^*) + \frac{\eta_t^2 \Bar{\sigma}^2}{n}  \\ 
	%& \hspace{1cm} + \eta_t^3 \left(  \frac{2L + \mu}{n}  \right) \frac{20A}{p^2}
	%\end{align}
	Substituting $A = 2nG^2 + \frac{p}{2}\left( \frac{8nG^2}{\omega} + \frac{5\omega n c_0}{4} \right)$ yields:
	\begin{align*}
	\mathbb{E} \Vert \Bar{x}^{(t+1)} - x^* \Vert^2 & \leq \left( 1-\frac{\eta_t \mu}{2} \right) \mathbb{E} \Vert \Bar{x}^{(t)} - x^* \Vert^2 - \eta_t (\mathbb{E}f(\Bar{x}^{(t)}) - f^*) + \frac{\eta_t^2 \Bar{\sigma}^2}{n} + \eta_t^3 \left(  \frac{2L + \mu}{n}  \right) \frac{20}{p^2}\left( 2nG^2 + \frac{p}{2}\left( \frac{8nG^2}{\omega} + \frac{5\omega n c_0}{4} \right) \right)
	\end{align*}
	We use Lemma \ref{suppl_cvx_lemma_stitch} for the sequence relation above by defining:
	\begin{align*}
	a_t & = \mathbb{E} \Vert \Bar{x}^{(t)} - x^* \Vert^2 \\
	e_t & = \mathbb{E}f(\Bar{x}^{(t)}) - f^* \\
	P & = 1 \\ 
	Q & = \frac{ \Bar{\sigma}^2}{n} \\
	R & = \left(  \frac{2L + \mu}{n}  \right) \frac{20}{p^2}\left( 2nG^2 + \frac{p}{2}\left( \frac{8nG^2}{\omega} + \frac{5\omega n c_0}{4} \right) \right)
	\end{align*}
	%Thus we get:
	%\begin{align*}
	%\frac{1}{S_T} \sum_{t=0}^{T-1}w_t e_t \leq \frac{\mu a^3}{8S_T}\Vert \bar{x}^{(0)} - x^* \Vert^2 + \frac{2T(T+2a)}{\mu S_T}\frac{ \Bar{\sigma}^2}{n} + \frac{16T}{\mu^2 S_T}\left(  \frac{2L + \mu}{n}  \right) \frac{20}{p^2}\left( 2nG^2 + \frac{pc_1}{2} \right)
	%\end{align*}
	%Substituting value of $c_1 = \frac{8nG^2}{\omega} + \frac{5\omega n c_0}{4}$ gives:
	For $w_t = (a+t)^2$, $a_0 =  \Vert \Bar{x}^{(0)} - x^* \Vert^2 $ and $e_t = \mathbb{E}f(\Bar{x}^{(t)}) - f^*$, this gives us the relation:
	\begin{align*}
	\frac{1}{S_T} \sum_{t=0}^{T-1}w_t e_t \leq \frac{\mu a^3}{8S_T}a_0 + \frac{2T(T+2a)}{\mu S_T}\frac{ \Bar{\sigma}^2}{n} + \frac{16T}{\mu^2 S_T}\left(  \frac{2L + \mu}{n}  \right) \frac{20}{p^2}\left( 2nG^2 + \frac{p}{2}\left(\frac{8nG^2}{\omega} + \frac{5\omega n c_0}{4} \right) \right)
	\end{align*}
	From the convexity of $f$, we have finally have: 
	\begin{align*}
	\mathbb{E}f(x_{avg}^{(T)}) - f^* \leq \frac{\mu a^3}{8S_T}a_0 + \frac{2T(T+2a)}{\mu S_T}\frac{ \Bar{\sigma}^2}{n} + \frac{16T}{\mu^2 S_T}\left(  \frac{2L + \mu}{n}  \right) \frac{20}{p^2}\left( 2nG^2 + \frac{p}{2}\left(\frac{8nG^2}{\omega} + \frac{5\omega n c_0}{4} \right) \right)
	\end{align*}
	%(where $e_t = f(\Bar{x}^{(t)}) - f^*$)
	where  $\Bar{x}^{(T)}_{avg} = \frac{1}{S_T} \sum_{t=0}^{T-1}w_t \bar{x}^{(t)}$.
	This completes the proof of Theorem \ref{thm_cvx}.
\end{proof}
%------------Lemma-------
\begin{lemma} \label{suppl_cvx_lemma_stitch}
	(From \cite{stich_sparsified_2018})
	Let $\{ a_t \}_{t \geq 0}, a_t \geq 0, e_t \}_{t \geq 0}, e_t \geq 0 $ be sequences satisfying :
	\begin{align*}
	a_{t+1} \leq (1-\mu \eta_t) a_{t} - \eta_t e_t P + \eta_t^2Q + \eta_t^3R,
	\end{align*}
	for stepsizes $\eta_t = \frac{4}{\mu (a+t)} $ and constants $P>0,Q,R \geq 0, \mu>0, a>1. $ Then :
	\begin{align*}
	\frac{P}{S_T} \sum_{t=0}^{T-1}w_t e_t \leq \frac{\mu a^3}{4S_T}a_0 + \frac{2T(T+2a)}{\mu S_T}Q + \frac{16T}{\mu^2 S_T}R,
	\end{align*}
	for $w_t = (a+t)^2$ and $S_T := \sum_{t=0}^{T-1}w_t = \frac{T}{6} (2T^2+6aT-3T+6a^2-6a+1) \geq \frac{1}{3}T^3$
\end{lemma}
%--------------------------------------------------------------------
%--------------------------------------------------------------------
\subsection{Proof of Theorem \ref{thm_noncvx_var} (Non-convex objective with varying step size)} \label{proof_thm_noncvx_var}
\begin{proof}[Proof of Theorem~\ref{thm_noncvx_var}:]
%	Considering the update rule as per (\ref{mean_seq_iter}) and taking expectation w.r.t sampling at timestep $t$ conditioned on the past:
%	\begin{align} \label{non_cvx_upd}
%	\mathbb{E}_{\xi_t} f(\bar{x}_{t+1}) & \stackrel{(\ref{mean_seq_iter})}{=} \mathbb{E}_{\xi_t} f \left(\bar{x}_{t} - \frac{\eta_t}{n}\sum_{j=1}^n \nabla F_j(x_t^{(j)},\xi_t^{(j)} ) \right) \notag \\
%	& \stackrel{(\ref{l_smooth})}{\leq } f(\bar{x}_{t}) - \mathbb{E}_{\xi_t} \left\langle \nabla f(\bar{x}_{t}) , \frac{\eta_t}{n}\sum_{j=1}^n \nabla F_j(x_t^{(j)},\xi_t^{(j)} ) \right\rangle + \mathbb{E}_{\xi_t} \frac{L}{2}\eta_t^2 \left\Vert \frac{1}{n}\sum_{j=1}^n \nabla F_j(x_t^{(j)},\xi_t^{(j)} ) \right\Vert_2^2
%	\end{align}
%	To estimate the second term in (\ref{non_cvx_upd}), we note that :
%	\begin{align} \label{non_cvx_upd_t1}
%	-\eta_t \mathbb{E}_{\xi_t} \left\langle \nabla f(\bar{x}_{t}) , \frac{1}{n}\sum_{j=1}^n \nabla F_j(x_t^{(j)},\xi_t^{(j)} ) \right\rangle & = - \eta_t \left\langle \nabla f(\bar{x}_{t}) , \frac{1}{n}\sum_{j=1}^n \nabla f_j(x_t^{(j)} ) \right\rangle \notag \\
%	& \stackrel{(c)}{=} - \eta_t  \Vert \nabla f(\bar{x}_{t})  \Vert_2^2 + \eta_t \left\langle \nabla f(\bar{x}_{t}) , \nabla f(\bar{x}_{t}) - \frac{1}{n}\sum_{j=1}^n \nabla f_j(x_t^{(j)}) \right\rangle \notag \\
%	& = - \eta_t  \Vert \nabla f(\bar{x}_{t})  \Vert_2^2 + \eta_t  \left\langle \nabla f(\bar{x}_{t}) ,  \frac{1}{n}\sum_{j=1}^n ( \nabla f_j(\bar{x}_{t}) - \nabla f_j(x_t^{(j)}) ) \right\rangle \notag \\
%	& \leq - \frac{\eta_t}{2}  \Vert \nabla f(\bar{x}_{t})  \Vert_2^2 + \frac{\eta_t}{2n}  \sum_{j=1}^n  \Vert \nabla f_j(\bar{x}_{t}) - \nabla f_j(x_t^{(j)}) \Vert^2
%	\end{align}
%	where in $(c)$ we add and subtract $\nabla f(\bar{x}_{t})$. To estimate the last term in (\ref{non_cvx_upd}), we add and subtract $\nabla f(\bar{x}_{t}) = \frac{1}{n}\sum_{j=1}^{n} \nabla f_i (\bar{x}_t ) $ and $\frac{1}{n}\sum_{j=1}^n \nabla f_j({x}_t^{(j)})$
%	\begin{align} \label{non_cvx_upd_t2}
%	 \frac{L}{2}\eta_t^2 \mathbb{E} _{\xi_t} \left\Vert \frac{1}{n}\sum_{j=1}^n \nabla F_j(x_t^{(j)},\xi_t^{(j)} ) \right\Vert_2^2 & = \mathbb{E} _{\xi_t} \left[ \frac{L}{2}\eta_t^2 \left\Vert \frac{1}{n}\sum_{j=1}^n (\nabla F_j(x_t^{(j)},\xi_t^{(j)} ) - \nabla f_j(x_t^{(j)} ) ) + \frac{1}{n}\sum_{j=1}^n (\nabla f_j(x_t^{(j)}) - \nabla f_j(\bar{x}_{t})) + \nabla f(\bar{x}_{t}) \right\Vert_2^2 \right] \notag \\
%%	& \leq  L\eta_t^2 \mathbb{E} _{\xi_t} \left\Vert \frac{1}{n}\sum_{j=1}^n (\nabla F_j(x_t^{(j)},\xi_t^{(j)} - \nabla f_j(x_t^{(j)} ) )  \right\Vert_2^2 + 2L\eta_t^2  \left\Vert \frac{1}{n}\sum_{j=1}^n (\nabla f_j(x_t^{(j)}) - \nabla f_j(\bar{x}_{t}))\right\Vert_2^2 \\
%%	& \hspace{2cm} + 2L\eta_t^2 \left\Vert \nabla f(\bar{x}_{t}) \right\Vert_2^2  \\
%	& \leq  L\eta_t^2 \mathbb{E} _{\xi_t} \left\Vert \frac{1}{n}\sum_{j=1}^n (\nabla F_j(x_t^{(j)},\xi_t^{(j)} - \nabla f_j(x_t^{(j)} ) )  \right\Vert_2^2 +  \frac{2L\eta_t^2}{n} \sum_{j=1}^n  \left\Vert  (\nabla f_j(x_t^{(j)}) - \nabla f_j(\bar{x}_{t}))\right\Vert_2^2 \notag  \\
%	& \hspace{2cm} + 2L\eta_t^2 \left\Vert \nabla f(\bar{x}_{t}) \right\Vert_2^2 \notag  \\
%%	\intertext{We can use the variance bound for the first term in (111) using the argument from (77)-(80) and noting that $\bar{\sigma}^2 = \frac{1}{n} \sum_{i=1}^n \sigma_i^2$:}
%	& \stackrel{(\ref{bound_var})}{\leq} \frac{L\eta_t^2 \bar{\sigma}^2}{n} +    \frac{2L\eta_t^2}{n} \sum_{j=1}^n \left\Vert  (\nabla f_j(x_t^{(j)}) - \nabla f_j(\bar{x}_{t}))\right\Vert_2^2 + 2L\eta_t^2 \left\Vert \nabla f(\bar{x}_{t}) \right\Vert_2^2   
%	\end{align}
%	Substituting (\ref{non_cvx_upd_t1}), (\ref{non_cvx_upd_t2}) to (\ref{non_cvx_upd}) gives:
%	\begin{align} \label{non_cvx_eqn_temp}
%	\mathbb{E} _{\xi_t} [f(\bar{x}_{t+1})] 
%%	& \leq   f(\bar{x}_{t}) - \frac{\eta_t}{2}  \Vert \nabla f(\bar{x}_{t})  \Vert_2^2 + \frac{\eta_t}{2n}  \sum_{j=1}^n   \Vert \nabla f_j(\bar{x}_{t}) - \nabla f_j(x_t^{(j)}) \Vert^2 + \frac{L\eta_t^2 \bar{\sigma}^2}{n} \\ 
%%	& \hspace{2cm} +  \frac{2L\eta_t^2}{n} \sum_{j=1}^n  \left\Vert  \nabla f_j(x_t^{(j)}) - \nabla f_j(\bar{x}_{t}) \right\Vert_2^2 + 2L\eta_t^2   \left\Vert  \nabla f(\bar{x}_{t}) \right\Vert_2^2 \\
%%	& \leq  f(\bar{x}_{t}) - \eta_t \left( \frac{1}{2} - 2L\eta_t \right)  \Vert \nabla f(\bar{x}_{t})  \Vert_2^2 + \left( \frac{\eta_t}{2n} + \frac{2L\eta_t^2}{n} \right) \sum_{j=1}^n \Vert \nabla f_j(\bar{x}_{t}) - \nabla f_j(x_t^{(j)}) \Vert^2 + \frac{L\eta_t^2 \bar{\sigma}^2}{n} \\
%%	\intertext{Using the L-smoothness of $f_j(x) \, \,  \forall j \in [n] $, we have:}
%	& \leq  f(\bar{x}_{t}) - \eta_t \left( \frac{1}{2} - 2L\eta_t \right)  \Vert \nabla f(\bar{x}_{t})  \Vert_2^2 + \left( \frac{\eta_tL}{2n} + \frac{2L^2\eta_t^2}{n} \right) \sum_{j=1}^n  \Vert \bar{x}_{t} - x_t^{(j)} \Vert^2 + \frac{L\eta_t^2 \bar{\sigma}^2}{n} 
%	\end{align}
	We now take expectation w.r.t the whole process and use Lemma \ref{lem_dec_sgd} to bound  $\sum_{j=1}^n \Vert \bar{x}_{t} - x_t^{(j)} \Vert^2$ :  
	\begin{align*}
	\mathbb{E} f(\bar{x}_{t+1}) & \leq \mathbb{E} f(\bar{x}_{t}) - \eta_t \left( \frac{1}{2} - 2L\eta_t \right) \mathbb{E} \Vert \nabla f(\bar{x}_{t})  \Vert_2^2 + \left( \frac{\eta_tL}{2n} + \frac{2L^2\eta_t^2}{n} \right) \frac{20\eta_t^2A}{p^2} + L\eta_t^2 \bar{\sigma}^2 
	\intertext{where $A= 2nG^2 + \frac{p}{2}\left( \frac{8nG^2}{\omega} + \frac{5\omega n c_0}{4} \right)$ . For the choice of $\eta_t = \frac{b}{(t+a)}$ and $a \geq \text{max} \left\{  \frac{5}{p}, 8bL  \right\}  $, we have $\eta_t \leq \frac{1}{8L}$: }
	& \leq \mathbb{E} f(\bar{x}_{t}) - \frac{\eta_t}{4} \mathbb{E} \Vert \nabla f(\bar{x}_{t})  \Vert_2^2 +  \frac{10LA}{np^2}\eta_t^3 + \frac{40L^2A}{np^2}\eta_t^4 + \frac{L\eta_t^2 \bar{\sigma}^2}{n}
	\end{align*}
	Rearranging the terms and summing from $0$ to $T-1$, we get:
	\begin{align} \label{non_cvx_rec_rel}
	\sum_{t=0}^{T-1} \eta_t  \mathbb{E} \Vert \nabla f(\bar{x}_{t}) \Vert_2^2  \leq 4 \left( f(\bar{x}_{0}) - \mathbb{E} f(\bar{x}_{T}) \right) +  \frac{40LA}{np^2} { \sum_{t=0}^{T-1}\eta_t^3} + \frac{160L^2A}{np^2}{ \sum_{t=0}^{T-1}\eta_t^4} + \frac{4L \bar{\sigma}^2}{n} {\sum_{t=0}^{T-1}\eta_t^2} \notag
	\intertext{Dividing both sides by $\sum_{t=0}^{T-1}\eta_t$ , we have:}
	\frac{\sum_{t=0}^{T-1} \eta_t  \mathbb{E} \Vert \nabla f(\bar{x}_{t}) \Vert_2^2}{{\sum_{t=0}^{T-1}\eta_t}}  \leq \frac{4 \left( f(\bar{x}_{0}) - \mathbb{E} f(\bar{x}_{T-1}) \right) }{\sum_{t=0}^{T-1}\eta_t} +  \frac{40LA}{np^2} \frac{ \sum_{t=0}^{T-1}\eta_t^3}{\sum_{t=0}^{T-1}\eta_t} + \frac{160L^2A}{np^2}\frac{ \sum_{t=0}^{T-1}\eta_t^4}{\sum_{t=0}^{T-1}\eta_t} + \frac{4L \bar{\sigma}^2}{n} \frac{\sum_{t=0}^{T-1}\eta_t^2}{\sum_{t=0}^{T-1}\eta_t}
	\end{align}
	We now note the following bounds on the sum of series $\eta_t = \frac{b}{t+a}$ :
	\begin{align*} 
	\sum_{t=0}^{T-1} \eta_t \geq \int_{0}^{T-1} \frac{b}{t+a} dt = b \log \left( \frac{T+a-1}{a} \right) \\
	\sum_{t=0}^{T-1} \eta_t^2 \leq \eta_0^2 + \int_{0}^{T-1} \frac{b^2}{(t+a)^2} dt  \leq \eta_0^2 + \int_{0}^{\inf} \frac{b^2}{(t+a)^2} dt = \eta_0^2 + \frac{b^2}{a} = \frac{b^2}{a^2} + \frac{b^2}{a}  \\
	\sum_{t=0}^{T-1} \eta_t^3 \leq \eta_0^3 + \int_{0}^{T-1} \frac{b^3}{(t+a)^3} dt  \leq \eta_0^3 + \int_{0}^{\inf} \frac{b^3}{(t+a)^3} dt = \eta_0^3 + \frac{b^3}{2a^2} = \frac{b^3}{a^3} + \frac{b^3}{2a^2} \\
	\sum_{t=0}^{T-1} \eta_t^4 \leq \eta_0^4 + \int_{0}^{T-1} \frac{b^4}{(t+a)^4} dt  \leq \eta_0^4 + \int_{0}^{\inf} \frac{b^4}{(t+a)^4} dt = \eta_0^3 + \frac{b^4}{3a^3} = \frac{b^4}{a^4} + \frac{b^4}{3a^3}
	\end{align*}
	Substituting these bounds in (\ref{non_cvx_rec_rel}) and noting that $\mathbb{E} f(\bar{x}_T) \geq f(x^*) = f^*  $   we get:
	\begin{align*}
	\frac{\sum_{t=0}^{T-1} \eta_t  \mathbb{E} \Vert \nabla f(\bar{x}_{t}) \Vert_2^2}{{\sum_{t=0}^{T-1}\eta_t}}  \leq \frac{4 \left( f(\bar{x}_{0}) - f^* \right) }{b \log \left( \frac{T+a-1}{a} \right)} +  \frac{40LA}{np^2} \frac{\left(\frac{b^3}{a^3} + \frac{b^3}{2a^2}\right)}{b \log \left( \frac{T+a-1}{a} \right)} + \frac{160L^2A}{np^2}\frac{ \left(\frac{b^4}{a^4} + \frac{b^4}{3a^3} \right)}{b \log \left( \frac{T+a-1}{a} \right)} + \frac{4L \bar{\sigma}^2}{n} \frac{\left(\frac{b^2}{a^2} + \frac{b^2}{a}\right)}{b \log \left( \frac{T+a-1}{a} \right)}
	\end{align*}
	where $A= 2nG^2 + \frac{p}{2}\left( \frac{8nG^2}{\omega} + \frac{5\omega n c_0}{4} \right)$. This completes proof of Theorem \ref{thm_noncvx_var} .
\end{proof} 
%--------------------------------------------------------------------
%--------------------------------------------------------------------
\subsection{Proof of Lemma \ref{lemm_dec_sgd_fix}} \label{proof_lemm_dec_sgd_fix}
\begin{lemma*} (Restating Lemma \ref{lemm_dec_sgd_fix} )
	Consider the sequence of updates as in Algorithm \ref{alg_dec_sgd} with some constant step size $\eta$. Then in matrix notation from Appendix \ref{mat_not_sec}, we have:
	\begin{align*}
	\mathbb{E}\sum_{j=1}^n \Vert \bar{x}_{t} - x_t^{(j)} \Vert^2 = \mathbb{E}\Vert\Bar{X}^{{(t)}} - X^{{(t)}}\Vert_F^2 \leq \frac{4A\eta^2}{p^2}
	\end{align*}
	where  $p = \frac{\delta^2 \omega}{644} $, $\delta := 1 - | \lambda_2(W)|$, $\omega$ is contraction parameter for quantization operator $Q$, $ A=2nG^2 + \frac{p}{2} \left( \frac{8nG^2}{\omega} + \frac{5\omega n c_0}{4} \right) $
\end{lemma*}
\begin{proof}[Proof of Lemma \ref{lemm_dec_sgd_fix}]
	We use the same steps for the Proof of Lemma \ref{lem_dec_sgd} wtih $\eta_t = \eta$, till eqn (\ref{suppl_lemm_rec_rel}). This gives us:
	\begin{align*} 
	\mathbb{E}[e_{t+1}] \leq \left( 1- \frac{p}{2} \right)\mathbb{E}[e_t] + \frac{2A}{p} \eta^2
	\end{align*}
	where   $e_{t+1} := \Vert X^{(t+1)} - \Bar{X}^{(t+1)} \Vert_F^2 + \Vert X^{(t+1)} - \hat{X}^{(t+2)} \Vert_F^2$ and  $A := 2nG^2 + \frac{p }{2}\left( \frac{8nG^2}{\omega} + \frac{5\omega n c_0}{4} \right) $. \\
	It can be seen that $\mathbb{E}[e_t] \leq \frac{4A}{p^2}\eta^2$ satisfies the recursion above. Using $\mathbb{E}[ \Vert X^{(t)} - \Bar{X}^{(t)} \Vert_F^2 ] \leq \mathbb{E}[e_t] $ completes the proof.
\end{proof}
%--------------------------------------------------------------------
%--------------------------------------------------------------------
\subsection{Proof of Theorem \ref{thm_noncvx_fix} (Non-convex objective with constant step size)} \label{proof_thm_noncvx_fix}
\begin{proof}[Proof of Theorem~\ref{thm_noncvx_fix}:]
The proof follows the same steps as Proof of Theorem \ref{thm_noncvx_var} till (\ref{non_cvx_eqn_temp}) with $\eta_t = \eta = \sqrt{\frac{n}{T}}$
\begin{align}
	\mathbb{E} _{\xi_t} [f(\bar{x}_{t+1})] 	& \leq  f(\bar{x}_{t}) - \eta \left( \frac{1}{2} - 2L\eta \right)  \Vert \nabla f(\bar{x}_{t})  \Vert_2^2 + \left( \frac{\eta L}{2n} + \frac{2L^2\eta^2}{n} \right) \sum_{j=1}^n  \Vert \bar{x}_{t} - x_t^{(j)} \Vert^2 + \frac{L\eta^2 \bar{\sigma}^2}{n} 
\end{align}
where $\xi_t$ denotes stochastic samples at timestep $t$. Taking expectation w.r.t the entire process and using Lemma \ref{lemm_dec_sgd_fix}:
%We use a modified version of Lemma 0.9. Specifically:
%\begin{align}
%e_{t+1} \leq \left( 1 - \frac{p}{2} \right) e_t + \frac{2A}{p} \eta^2
%\end{align}
%It can be easily seen that $e_t \leq \frac{4A}{p^2}\eta^2$ satisfies the recursion and thus the difference is in bounding the term $\Gamma_t = \Vert X^{(t)} - \bar{X}^{(t)} \Vert_F^2 $ as $\Gamma_t \leq \frac{4A}{p^2}\eta^2 $. \\
%Thus the proof proceeds as:
\begin{align*}
\mathbb{E} f(\bar{x}_{t+1}) & \leq \mathbb{E} f(\bar{x}_{t}) - \eta \left( \frac{1}{2} - 2L\eta \right) \mathbb{E} \Vert \nabla f(\bar{x}_{t})  \Vert_2^2 + \left( \frac{\eta L}{2n} + \frac{2L^2\eta^2}{n} \right) \frac{4\eta^2A}{p^2} + \frac{L\bar{\sigma}^2\eta^2}{n}
\intertext{where $A := 2nG^2 + \frac{p }{2}\left( \frac{8nG^2}{\omega} + \frac{5\omega n c_0}{4} \right) $ . For the choice of $\eta = \sqrt{\frac{n}{T}}$ and $T \geq 64nL^2$, we have $\eta \leq \frac{1}{8L}$, which gives:}
& \leq \mathbb{E} f(\bar{x}_{t}) - \frac{\eta}{4} \mathbb{E} \Vert \nabla f(\bar{x}_{t})  \Vert_2^2 +  \frac{2LA}{np^2}\eta^3 + \frac{8L^2A}{np^2}\eta^4 + \frac{L\bar{\sigma}^2\eta^2}{n} 
\end{align*}
Rearranging the terms and summing from $0$ to $T-1$, we get:
\begin{align*}
\sum_{t=0}^{T-1} \eta  \mathbb{E} \Vert \nabla f(\bar{x}_{t}) \Vert_2^2  \leq 4 \left( f(\bar{x}_{0}) - \mathbb{E} f(\bar{x}_{T}) \right) +  \frac{8LA}{np^2} { \sum_{t=0}^{T-1}\eta^3} + \frac{32L^2A}{np^2}{ \sum_{t=0}^{T-1}\eta^4} + \frac{4L\bar{\sigma}^2}{n} {\sum_{t=0}^{T-1}\eta^2}
\end{align*}
Dividing both sides by $\sum_{t=0}^{T-1}\eta$, we finally have:
\begin{align}
%\frac{\sum_{t=0}^{T-1} \eta  \mathbb{E} \Vert \nabla f(\bar{x}_{t}) \Vert_2^2}{{\sum_{t=0}^{T-1}\eta}}  
%& \leq \frac{4 \left( f(\bar{x}_{0}) - \mathbb{E} f(\bar{x}_{T-1}) \right) }{\sum_{t=0}^{T-1}\eta} +  \frac{8LA}{np^2} \frac{ \sum_{t=0}^{T-1}\eta^3}{\sum_{t=0}^{T-1}\eta} + \frac{32L^2A}{np^2}\frac{ \sum_{t=0}^{T-1}\eta^4}{\sum_{t=0}^{T-1}\eta} + \frac{4L\bar{\sigma}^2}{n} \frac{\sum_{t=0}^{T-1}\eta^2}{\sum_{t=0}^{T-1}\eta} \\
%\end{align}
%\begin{align}
%\frac{\sum_{t=0}^{T-1}  \mathbb{E} \Vert \nabla f(\bar{x}_{t}) \Vert_2^2}{T}
\frac{\sum_{t=0}^{T-1}  \mathbb{E} \Vert \nabla f(\bar{x}_{t}) \Vert_2^2}{T}  \leq \frac{4 \left( f(\bar{x}_{0}) - f^*) \right) }{\eta T} +  \frac{8LA}{np^2} \eta^2 + \frac{32L^2A}{np^2}\eta^3 + \frac{4L\bar{\sigma}^2}{n} \eta
\end{align}
where $A= 2nG^2 + \frac{p }{2}\left( \frac{8nG^2}{\omega} + \frac{5\omega n c_0}{4} \right)$. Substituting $\eta = \sqrt{\frac{n}{T}}$ completes the proof.
\end{proof}
